Physico-chemical Processes in Planet-forming Discs

This thesis summarises my scientific works in the field of thermo-chemical modelling of planet-forming discs since 2009, in particular the development of the Protoplanetary Disc Model (ProDiMo). By combining chemical rate networks with continuum & line radiative transfer, and the calculation of all relevant dust and gas heating & cooling rates in an axisymmetric disc structure, these models make detailed predictions about the molecular composition of the disc, the discs' internal gas and dust temperature structure, and the composition of ice layers which form on the refractory dust grain surfaces. The development of ProDiMo was a process that took about 15 years. I have started the ProDiMo project and am the main developer, but without the involvement of an international team of scientists, in particular Inga Kamp, Wing-Fai Thi and Christian Rab, ProDiMo would not have its capabilities and would not be at the level of international recognition that is has achieved to date. Using formal solutions of the line & continuum radiative transfer, we can predict the spectral appearance of these discs from optical to millimetre wavelengths, for example the continuum and line fluxes, monochromatic images, radial intensity profiles, high-resolution line profiles that probe the disc dynamics, visibilities and channel maps. A large part of this thesis describes the publications that compared these predictions to disc observations that have been obtained by various space-borne and ground-based astronomical instruments, in particular Herschel/PACS, Spitzer/IRS, VLT/CRIRES, JWST/MIRI and ALMA. These observations probe the gas and the dust in different radial disc regions and in different layers above the midplane. This thesis summarises the conclusions drawn from the ProDiMo thermo-chemical disc models about the chemical and physical state of protoplanetary discs as the birth places of exoplanets.

==> my_headers.tex <==
%
%   Hier folgen meine Definitionen fuer header und footer-Gestaltung
%
%  Benoetigt: package fancyheadings
%
%\usepackage{fancyheadings}% braucht man, um header flexibel zu setzten.
%\pagestyle{fancy}%  falls nicht twoside
\pagestyle{fancyplain}% falls twoside
%
\newcommand{\mottostyle}{\sf\footnotesize}% Stil fuer Motti 
                                          % bei neuen Kapiteln

\renewcommand{\sectionmark}[1]{\markboth{\sectionname\
                                         \thesection. #1}{}}
\renewcommand{\sectionmark}[1]{\markright{\thesection. #1}}
%\renewcommand{\chaptermark}[1]% gibt headerschrift nicht in Kapitaelchen
%{\markboth{#1}{}}             % Warum???
%\renewcommand{\sectionmark}[1]%
%{\markright{\thesection\ #1}}
%
%\lhead[]{}%  hier ist das optionale Argument immer fuer gerade (linke)
%\chead[]{}%  Seiten
%\rhead[]{}
%\lfoot[]{}
%\cfoot[]{}
%\rfoot[]{}
% hier folgen die Definitionen, die man benutzen sollte,
% falls man twoside benutzt mit \pagestyle{fancyplain}\lhead[]{}   
%
% man benutze: \fancyplain{plain_value}{normal_value}
% in den einzelnen Argumenten !
\lhead[\fancyplain{}{\rm\thepage}]{\fancyplain{}{\sf\scriptsize\rightmark}}
%\chead[\fancyplain{\sf\scriptsize\today\ \printtime}
%{\sf\scriptsize\today\ \printtime}]
%{\fancyplain{\sf\scriptsize\today\ \printtime}
%{\sf\scriptsize\today\ \printtime}}
\newcommand{\motto}{}% Brauche ich fuer das Motto eines Kapitels:
%                      Direkt vor \chapter[]{} definiere man um:
% \renewcommand{\motto}{Hier das Motto des Kapitels}
\rhead[\fancyplain{}{\sf\scriptsize\leftmark}]%
{\fancyplain{\vspace{20mm}\mottostyle\motto}{\rm\thepage}}
\lfoot[\fancyplain{}{}]{\fancyplain{}{}}        
\cfoot[\fancyplain{}{}]{\fancyplain{\rm\thepage}{}}
\rfoot[\fancyplain{}{}]{\fancyplain{}{}}
%\setlength{\headrulewidth}{}% default: 0.4pt
%\setlength{\footrulewidth}{}% default: 0pt
\setlength{\plainheadrulewidth}{0.4pt} % die gleichen Werte fuer plain-pages,
%\setlength{\plainfootrulewidth}{} % die verwendet werden, falls automatisch
%                                 in plain-modus geschaltet wird, etwa bei
%                                 \chapter (\section) oder \thispagestyle
%\setlength{\headwidth}{} % default: \textwidth Breite fuer header UND footer
%\setlength{\headheigth}{}   % muss man aendern, falls header oder footer
%\setlength{\footskip}{}     % zu gross werden; eventuell fuer Motti !
%\addtolength{\headheigth}{}
%\addtolength{\footskip}{}
%\addtolength{\headwidth}{\marginparsep}
%\addtolength{\headwidth}{\marginparwidth}











==> pdfs.tex <==
\section*{\bff Publication 7:}
\addcontentsline{toc}{section}{\bff Publication 7}  



